Im2Hands: Learning Attentive Implicit Representation of Interacting Two-Hand Shapes

We present Implicit Two Hands (Im2Hands), the first neural implicit representation of two interacting hands. Unlike existing methods on two-hand reconstruction that rely on a parametric hand model and/or low-resolution meshes, Im2Hands can produce fine-grained geometry of two hands with high hand-to-hand and hand-to-image coherency. To handle the shape complexity and interaction context between two hands, Im2Hands models the occupancy volume of two hands - conditioned on an RGB image and coarse 3D keypoints - by two novel attention-based modules responsible for (1) initial occupancy estimation and (2) context-aware occupancy refinement, respectively. Im2Hands first learns per-hand neural articulated occupancy in the canonical space designed for each hand using query-image attention. It then refines the initial two-hand occupancy in the posed space to enhance the coherency between the two hand shapes using query-anchor attention. In addition, we introduce an optional keypoint refinement module to enable robust two-hand shape estimation from predicted hand keypoints in a single-image reconstruction scenario. We experimentally demonstrate the effectiveness of Im2Hands on two-hand reconstruction in comparison to related methods, where ours achieves state-of-the-art results. Our code is publicly available at https://github.com/jyunlee/Im2Hands.

==> tables/table_rebuttal_ablation.tex <==
\begin{table}[!h]
\centering
{ \footnotesize
\setlength{\tabcolsep}{0.2em}
\renewcommand{\arraystretch}{1.0}
\caption{\textbf{Results of additional ablation study using the \emph{predicted} keypoints of DIGIT~[11].}}
\label{table:rebuttal_ablation}
\vspace{-0.4\baselineskip}
\begin{tabularx}{\columnwidth}{>{\centering}m{4.8cm}|Y|Y}
\toprule
Method & IoU \footnotesize{(\%)} $\uparrow$ & CD \footnotesize{(mm)} $\downarrow$ \\
\midrule
$\mathcal{K} + \mathcal{I}$ & 55.4 & 7.61 \\
$\mathcal{K} + \mathcal{I}$ + $\mathcal{R}$ - $\mathrm{FeatureCloud}$ & 58.3 & 4.78 \\
$\mathcal{K} + \mathcal{I}$ + $\mathcal{R}$ - $\mathrm{ContextLatent}$ & 58.4 & 4.79 \\
\midrule
\textbf{Im2Hands ($\mathcal{K}$ + $\mathcal{I}$ + $\mathcal{R}$)} & \textbf{59.4} & \textbf{4.75} \\ 
\bottomrule
\end{tabularx}
}
\vspace{-0.6\baselineskip}
\end{table}

==> tables/table_rebuttal_intersec.tex <==
\begin{table}[!h]
\centering
{ \footnotesize
\setlength{\tabcolsep}{0.2em}
\renewcommand{\arraystretch}{1.0}
\caption{ \textbf{Difference in intersection volume and depth with the GT.}  For intersection depth, we measured L1-difference.}
\label{table:rebuttal_intersec}
\vspace{-0.5\baselineskip}
\begin{tabularx}{\columnwidth}{>{\centering}m{3cm}|Y|Y}
\toprule
Method & Volume diff. (cm$^3$) & Depth diff. (mm) \\
\midrule
IntagHand~[23] & 14.14 & 0.13 \\
\textbf{Im2Hands (Ours)} & \textbf{8.78} & \textbf{0.09} \\ 
\bottomrule
\end{tabularx}
}
\vspace{-0.5\baselineskip}
\end{table}
